A Fast Algorithm for Separated Sparsity via Perturbed Lagrangians

Sparsity-based methods are widely used in machine learning, statistics, and signal processing. There is now a rich class of structured sparsity approaches that expand the modeling power of the sparsity paradigm and incorporate constraints such as group sparsity, graph sparsity, or hierarchical sparsity. While these sparsity models offer improved sample complexity and better interpretability, the improvements come at a computational cost: it is often challenging to optimize over the (non-convex) constraint sets that capture various sparsity structures. In this paper, we make progress in this direction in the context of separated sparsity -- a fundamental sparsity notion that captures exclusion constraints in linearly ordered data such as time series. While prior algorithms for computing a projection onto this constraint set required quadratic time, we provide a perturbed Lagrangian relaxation approach that computes provably exact projection in only nearly-linear time. Although the sparsity constraint is non-convex, our perturbed Lagrangian approach is still guaranteed to find a globally optimal solution. In experiments, our new algorithms offer a 10$\times$ speed-up already on moderately-size inputs.

==> 375-reuse-it-maybe.tex <==
\subsection{Our approach}
At a high-level, we develop our algorithms in four main steps. We start (Section~\ref{sec:dual}) by considering the dual LP of $\LPdeltaprimal$ and show that its combinatorial structure can be exploited to compute an optimal solution to it in nearly-linear time.
More precisely, if $\ustar$ is an indicator vector of an optimal solution to $\LPdeltaprimal$
%, i.e., $\ustar_i = 1$ if $i$ is part of some (fixed) optimal solution, and $\ustar_i = 0$ otherwise,
we show how to compute $\left(\ustar\right)^T c$ in nearly-linear time.
By strong duality, this optimal dual solution gives us then the \emph{value} of the optimal primal solution. 

Second, in Section~\ref{subsec:active-constraints} we analyze properties of the dual LP and exhibit very close ties between its structure, as captured by so-called ``active constraints'', and the sparsity distribution of $\LPdeltaprimal$. These findings allow us to reason about the optimality of $\LPdeltaprimal$ in an alternative way, which we turn into two efficient algorithms -- a deterministic and a randomized.


We demonstrate that by analyzing answers of the dual oracle on perturbed versions of the original problem we can quickly recover a single non-zero entry of the optimal primal solution. This gives rise to our deterministic divide-and-conquer procedure that we sketch in Section~\ref{section:recover-delta}.

Widely applied approach in solving LP problems is to handle the ``hard'' constraints via Lagrangian relaxation. However, such approaches usually do not lead to solutions corresponding to the original problem. Our further study of the structure of dual LP allows us to formalize the cases in which the LP obtained after relaxing the sparsity constraint of $\LPdeltaprimal$ does not solution-wise coincide with $\LPdeltaprimal$. Furthermore, we show that those cases can be avoided by careful perturbation of the original instance. Building on these idea, we develop a randomized algorithm described in Section~\ref{sec:randomized}.


%\begin{table*}[ht]
%    \begin{center}
%        \begin{small}
%        \begin{sc}
%        \begin{tabular}{lcc}
%        \hline
%        \abovespace\belowspace
%        Reference & Running time & Measurement complexity \\
%        \hline
%        \abovespace
%        FILL-IN & $O(d \log{d})$ & $O(k \log{(d/k)}$ \\
%        \cite{hegdeLP} & $O(d^{3.5})$ & $O(k \log{(d/k - \Delta)})$ \\
%        \cite{FMN15} & $O(d^2)$ & $O(k \log{(d/k - \Delta)})$ \\
%        Section~\ref{sec:randomized} & $O(d\log{(\cmax + d)})$ & $O(k \log{(d/k - \Delta)})$ \\
%        \belowspace
%        Appendix~\ref{sec:dp}   & $O(d + k^2)$ & $O(k)^\star$ \\
%        \hline
%        \end{tabular}
%        \end{sc}
%        \end{small}
%    \end{center}
%    \vskip -0.1in
%    \caption{An overview on the past work and our result on $\Delta$-separated sparsity. The last row holds in the regime $d/k - \Delta \in O(1)$. Without loss of generality we assume $c$ is positive integral and $\cmax > 2$ (see Section~\ref{sec:lpperspective} for details).}
%    \label{table:overview}
%\end{table*}

==> 970-experiments-old.tex <==
\section{Experiments}
\label{app:experiments-old}


We now report initial experimental results for a variant of our algorithm described in Section \ref{sec:recoverprimal}.
While the stated algorithm $\recoverprimal(\mc, \mk)$ runs in nearly-linear time, its time complexity contains three logarithmic factors, which can be a disadvantage in practice.
To address this issue, we give an algorithm inspired by our greedy dual oracle and the active set analysis that only has a single logarithmic factor in its time complexity.

\subsection{Experimental algorithm}
At a high level, our algorithm consists of two parts.
Similar to the greedy dual oracle, we introduce a special variable $\lambda \in \bbR$.
We are interested in solving the following relaxed version of the original separated sparsity problem:
\begin{equation}
\label{eq:lagrangian}
    \min_{\Omega \in \Msupports_\Delta} \norm{c - c_\Omega}^2 + \lambda \abs{\Omega}
\end{equation}
where we write $\Msupports_\Delta$ for the set of $\Delta$-separated support patterns \emph{without} cardinality constraint.
For a fixed value of $\lambda$, we can solve this problem in linear time by considering the modified vector $c'_i = c_i^2 - \lambda$ and finding the best $\Delta$-separated approximation for this vector where we again ignore the cardinality constraint.

In this formulation, the parameter $\lambda$ essentially controls the trade-off between sparsity and approximation error:
a larger value of $\lambda$ leads to solutions of smaller size, while a smaller value of $\lambda$ penalizes large support patterns less and hence gives solutions of larger size.
By performing a binary search over $\lambda$, we can find a suitable trade-off parameter that corresponds to our desired sparsity with a logarithmic number of invocations to Problem \eqref{eq:lagrangian}.
Overall, this leads to a nearly-linear running time with only a single logarithmic factor.

We remark that the argument above only sketches correctness: while it is easy to see that the returned solution is indeed optimal for its sparsity value, a priori it is not clear that every target sparsity $k$ has a corresponding setting of the trade-off parameter $\lambda_k$.
We defer a formal discussion of this issue to the full version of the paper and focus on the empirical performance of the algorithm here.

\subsection{Results}
We compare our experimental algorithm outlined above with the $O(nk)$-time dynamic program described in Section \ref{sec:dp} as a baseline.
Note that this DP already has a better time complexity than the best previously known algorithm from \cite{FMN15}.
We have implemented both algorithms in the Julia programming language\footnote{\url{http://julialang.org/}} (version 0.4.2), which typically achieves performance close to C/C++ for combinatorial algorithms.
All experiments were conducted on a laptop computer with a 2.8 GHz Intel Core i7 CPU and 16 GB of RAM.

We use synthetic data as input for the algorithms.
For a problem size $n$, we first generate a random separated sparse vector with parameters $\Delta = 20$ and $k \approx 0.04n$.
The non-zero coefficients are i.i.d.\ $\pm 1$.
We then add Gaussian noise with $\sigma = 1/2$ to all coordinates.
In the following experiments, we vary the problem size from $n=10^3$ to $n=10^5$ and run ten independent trials for each combination of algorithm and problem size.

Figure \ref{fig:results} summarizes the results of our experiments.
The data clearly shows that our algorithm scales significantly better with the problem size and achieves a nearly-linear running time.
As predicted, the empirical time complexity of the dynamic program is essentially quadratic in the $k = O(n)$ regime we consider here.
For problem size $n=10^5$, our algorithm is more than two orders of magnitude faster.

\begin{figure}
\centering
\begin{tikzpicture}
\begin{loglogaxis}[title=Absolute running time,timeplot,name=timeplot1,ymax=10,ymin=0.0001]
\addplot table[x=n, y=time_mean, y error=time_std] {experiment1_lagrange.txt};
\addplot table[x=n, y=time_mean, y error=time_std] {experiment1_DP.txt};
\legend{Our algorithm,Dynamic program}
\end{loglogaxis}

\begin{loglogaxis}[title=Relative speed-up,timeratioplot,name=timeratioplot1,at=(timeplot1.north east),anchor=north west,xshift=\plotxspacing,ignore legend]
\addplot table[x=n, y=time_ratio] {experiment1_lagrange.txt};
\end{loglogaxis}
\end{tikzpicture}
\caption{Experimental results: the running time of our algorithm scales significantly better with the problem size $n$.
For $n=10^5$, our algorithm is more than two orders of magnitude faster than the dynamic program.}
\label{fig:results}
\end{figure}
